Electronic Appendix to "Input Invariants"

In this electronic appendix to our paper "Input Invariants," accepted at ESEC/FSE'22, we provide additional examples, formal definitions, theorems, and proof sketches to complement our paper. Furthermore, we show the invariants that ISLearn mined in our evaluation.

==> xx.tex <==


